Two-Timescale Transmission Design and RIS Optimization for Integrated Localization and Communications

Reconfigurable intelligent surfaces (RISs) have tremendous potential to boost communication performance, especially when the line-of-sight (LOS) path between the user equipment (UE) and base station (BS) is blocked. To control the RIS, channel state information (CSI) is needed, which entails significant pilot overhead. To reduce this overhead and the need for frequent RIS reconfiguration, we propose a novel framework for integrated localization and communications, where RIS configurations are fixed during location coherence intervals, while BS precoders are optimized every channel coherence interval. This framework leverages accurate location information obtained with the aid of several RISs as well as novel RIS optimization and channel estimation methods. Performance in terms of localization accuracy, channel estimation error, and achievable rate demonstrates the effectiveness of the proposed approach.

==> Figures_EPS/AR_Movement.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{every tick label/.append style={font=\footnotesize}}

\begin{tikzpicture}

\begin{axis}[%
width=0.95\textwidth,
height=0.45\textwidth,
at={(2,1.5)},
scale only axis,
xmin=0.5,
xmax=2,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Time in movement (s)},
ymin=1,
ymax=4.5,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize Conditional achievable rate (bits/s/Hz)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.5	4.23404813160297\\
1	3.89804418996836\\
1.5	3.65022658352861\\
2	3.4868733956429\\
};\label{Opt_P1}
\addplot [color=red, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.5	4.08907800421152\\
1	3.76687723415533\\
1.5	3.54732581262476\\
2	3.38060195422727\\
};\label{Opt_P1_Loc}
\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.5	2.09386376143982\\
1	2.08947182481116\\
1.5	2.08468057094031\\
2	2.08105245765572\\
};\label{OptPri}
\addplot [color=blue, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.5	1.72627603551676\\
1	1.72128589490398\\
1.5	1.71614391602111\\
2	1.7105068489438\\
};\label{OptPri_Loc}

\end{axis}
\node (Box1) [draw=none,fill=none] at (1, 3) {\shortstack[l]{ 
\ref{Opt_P1} \footnotesize (a) \\
\ref{OptPri} \footnotesize (b) \\
\ref{Opt_P1_Loc} \footnotesize (c) \\
\ref{OptPri_Loc} \footnotesize (d)
}};
\end{tikzpicture}%

==> Figures_EPS/CDF_AR.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor3}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor4}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{ForestGreen}{RGB}{34,139,34}
%
\pgfplotsset{every tick label/.append style={font=\footnotesize}}

\begin{tikzpicture}

\begin{axis}[%
width=0.95\textwidth,
height=0.45\textwidth,
at={(2,0.5)},
scale only axis,
xmin=0,
xmax=6,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Instantaneous achievable rate (bits/s/Hz) of UE 2},
ymode=log,
ymin=0.1,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize Cumulative distribution function},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.0642	0.000833333333333333\\
0.0654	0.00166666666666667\\
0.0666	0.00333333333333333\\
0.0678	0.00333333333333333\\
0.069	0.00416666666666667\\
0.0702	0.00666666666666667\\
0.0714	0.0075\\
0.0726	0.00833333333333333\\
0.0738	0.01\\
0.075	0.0175\\
0.0762	0.0258333333333333\\
0.0774	0.0308333333333333\\
0.0786	0.0391666666666667\\
0.0798	0.0533333333333333\\
0.081	0.0691666666666667\\
0.0822	0.09\\
0.0834	0.105833333333333\\
0.0846	0.124166666666667\\
0.0858	0.154166666666667\\
0.087	0.183333333333333\\
0.0882	0.209166666666667\\
0.0894	0.24\\
0.0906	0.288333333333333\\
0.0918	0.318333333333333\\
0.093	0.355833333333333\\
0.0942	0.395833333333333\\
0.0954	0.445\\
0.0966	0.495833333333333\\
0.0978	0.5375\\
0.099	0.575833333333333\\
0.1002	0.6225\\
0.1014	0.6625\\
0.1026	0.7125\\
0.1038	0.7525\\
0.105	0.775\\
0.1062	0.81\\
0.1074	0.831666666666667\\
0.1086	0.855\\
0.1098	0.876666666666667\\
0.111	0.893333333333333\\
0.1122	0.911666666666667\\
0.1134	0.923333333333333\\
0.1146	0.935\\
0.1158	0.951666666666667\\
0.117	0.964166666666667\\
0.1182	0.971666666666667\\
0.1194	0.9775\\
0.1206	0.98\\
0.1218	0.981666666666667\\
0.123	0.983333333333334\\
0.1242	0.985833333333333\\
0.1254	0.989166666666667\\
0.1266	0.990833333333333\\
0.1278	0.995\\
0.129	0.9975\\
0.1302	0.9975\\
0.1314	0.9975\\
0.1326	0.998333333333333\\
0.1338	0.998333333333333\\
0.135	1\\
};\label{Scheme1}

\addplot [color=black, dashdotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.075	0.0799333333333333\\
0.15	0.0876083333333333\\
0.225	0.118566666666667\\
0.3	0.126683333333333\\
0.375	0.139241666666667\\
0.45	0.19255\\
0.525	0.234716666666667\\
0.6	0.258916666666667\\
0.675	0.26005\\
0.75	0.270666666666667\\
0.825	0.28165\\
0.9	0.303908333333333\\
0.975	0.319591666666667\\
1.05	0.32\\
1.125	0.321241666666667\\
1.2	0.330075\\
1.275	0.341108333333333\\
1.35	0.369716666666667\\
1.425	0.404083333333333\\
1.5	0.412991666666667\\
1.575	0.420266666666667\\
1.65	0.437025\\
1.725	0.459158333333333\\
1.8	0.464925\\
1.875	0.499241666666667\\
1.95	0.545891666666667\\
2.025	0.550033333333333\\
2.1	0.570041666666667\\
2.175	0.612391666666667\\
2.25	0.637675\\
2.325	0.645825\\
2.4	0.659058333333333\\
2.475	0.669058333333333\\
2.55	0.682425\\
2.625	0.7053\\
2.7	0.741608333333333\\
2.775	0.753683333333333\\
2.85	0.76\\
2.925	0.761625\\
3	0.781808333333333\\
3.075	0.807791666666666\\
3.15	0.811916666666667\\
3.225	0.846741666666667\\
3.3	0.850583333333333\\
3.375	0.86\\
3.45	0.861966666666666\\
3.525	0.896516666666666\\
3.6	0.918666666666666\\
3.675	0.93\\
3.75	0.95\\
3.825	0.95\\
3.9	0.96\\
3.975	0.96\\
4.05	0.97\\
4.125	0.98\\
4.2	0.98\\
4.275	0.98\\
4.35	0.98945\\
4.425	0.99\\
4.5	1\\
};\label{Scheme2}

\addplot [color=magenta, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3.2015	0.000116666666666667\\
3.243	0.0125833333333333\\
3.2845	0.028875\\
3.326	0.0506916666666667\\
3.3675	0.0599583333333333\\
3.409	0.0697333333333333\\
3.4505	0.0710583333333333\\
3.492	0.08\\
3.5335	0.08\\
3.575	0.08\\
3.6165	0.08\\
3.658	0.08\\
3.6995	0.0808666666666667\\
3.741	0.0898416666666667\\
3.7825	0.09\\
3.824	0.105733333333333\\
3.8655	0.1109\\
3.907	0.152241666666667\\
3.9485	0.180175\\
3.99	0.193983333333333\\
4.0315	0.21\\
4.073	0.22\\
4.1145	0.22\\
4.156	0.221825\\
4.1975	0.23\\
4.239	0.235066666666667\\
4.2805	0.268891666666667\\
4.322	0.2966\\
4.3635	0.3\\
4.405	0.3157\\
4.4465	0.330575\\
4.488	0.363733333333333\\
4.5295	0.382708333333333\\
4.571	0.4\\
4.6125	0.420616666666667\\
4.654	0.46\\
4.6955	0.519425\\
4.737	0.55\\
4.7785	0.573625\\
4.82	0.601241666666667\\
4.8615	0.659975\\
4.903	0.693283333333333\\
4.9445	0.749325\\
4.986	0.778641666666667\\
5.0275	0.806675\\
5.069	0.828991666666667\\
5.1105	0.85\\
5.152	0.8683\\
5.1935	0.89\\
5.235	0.902616666666667\\
5.2765	0.91\\
5.318	0.92\\
5.3595	0.949958333333333\\
5.401	0.96\\
5.4425	0.96\\
5.484	0.96025\\
5.5255	0.97\\
5.567	0.97\\
5.6085	0.988925\\
5.65	1\\
};\label{Scheme3_10}

\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3.8095	0.000916666666666667\\
3.839	0.025\\
3.8685	0.025\\
3.898	0.025\\
3.9275	0.02875\\
3.957	0.0498958333333333\\
3.9865	0.050625\\
4.016	0.0719791666666667\\
4.0455	0.075\\
4.075	0.075\\
4.1045	0.075\\
4.134	0.075\\
4.1635	0.075\\
4.193	0.075\\
4.2225	0.075\\
4.252	0.075\\
4.2815	0.075\\
4.311	0.075\\
4.3405	0.075\\
4.37	0.075\\
4.3995	0.075\\
4.429	0.0856666666666667\\
4.4585	0.1\\
4.488	0.1\\
4.5175	0.125520833333333\\
4.547	0.150041666666667\\
4.5765	0.221708333333333\\
4.606	0.225\\
4.6355	0.225\\
4.665	0.249979166666667\\
4.6945	0.25\\
4.724	0.25\\
4.7535	0.275\\
4.783	0.275\\
4.8125	0.275\\
4.842	0.3235\\
4.8715	0.325020833333333\\
4.901	0.374520833333333\\
4.9305	0.375\\
4.96	0.383229166666667\\
4.9895	0.4\\
5.019	0.467541666666667\\
5.0485	0.504104166666667\\
5.078	0.575770833333333\\
5.1075	0.6000625\\
5.137	0.630083333333333\\
5.1665	0.689625\\
5.196	0.744979166666667\\
5.2255	0.824229166666667\\
5.255	0.875\\
5.2845	0.875\\
5.314	0.9\\
5.3435	0.911\\
5.373	0.925\\
5.4025	0.925\\
5.432	0.94725\\
5.4615	0.95\\
5.491	0.974375\\
5.5205	0.975\\
5.55	1\\
};\label{Scheme3_30}

\addplot [color=ForestGreen, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
5.355684	0.000833333333333333\\
5.355968	0.00166666666666667\\
5.356252	0.00166666666666667\\
5.356536	0.00166666666666667\\
5.35682	0.0025\\
5.357104	0.0025\\
5.357388	0.00583333333333333\\
5.357672	0.00833333333333333\\
5.357956	0.0141666666666667\\
5.35824	0.0158333333333333\\
5.358524	0.0183333333333333\\
5.358808	0.02\\
5.359092	0.025\\
5.359376	0.0316666666666667\\
5.35966	0.0391666666666667\\
5.359944	0.0491666666666667\\
5.360228	0.0591666666666667\\
5.360512	0.0741666666666667\\
5.360796	0.0941666666666667\\
5.36108	0.125833333333333\\
5.361364	0.1575\\
5.361648	0.186666666666667\\
5.361932	0.218333333333333\\
5.362216	0.245833333333333\\
5.3625	0.28\\
5.362784	0.314166666666667\\
5.363068	0.35\\
5.363352	0.389166666666667\\
5.363636	0.433333333333333\\
5.36392	0.474166666666667\\
5.364204	0.523333333333333\\
5.364488	0.563333333333333\\
5.364772	0.605\\
5.365056	0.653333333333333\\
5.36534	0.686666666666667\\
5.365624	0.723333333333333\\
5.365908	0.756666666666667\\
5.366192	0.794166666666667\\
5.366476	0.82\\
5.36676	0.839166666666667\\
5.367044	0.8625\\
5.367328	0.8875\\
5.367612	0.904166666666667\\
5.367896	0.923333333333333\\
5.36818	0.9425\\
5.368464	0.953333333333333\\
5.368748	0.968333333333333\\
5.369032	0.970833333333333\\
5.369316	0.976666666666667\\
5.3696	0.979166666666667\\
5.369884	0.986666666666667\\
5.370168	0.99\\
5.370452	0.993333333333333\\
5.370736	0.994166666666667\\
5.37102	0.995833333333333\\
5.371304	0.995833333333333\\
5.371588	0.996666666666667\\
5.371872	0.998333333333333\\
5.372156	0.998333333333333\\
5.37244	1\\
};\label{Scheme4}

\end{axis}

\node (Box1) [draw=none,fill=white] at (4, 2.3) {\shortstack[l]{ 
\ref{Scheme1} \footnotesize {Scheme 1}\\
\ref{Scheme2} \footnotesize {Scheme 2}\\
\ref{Scheme4} \footnotesize {Scheme 4}\\
\ref{Scheme3_10} \footnotesize {Scheme 3: $T_{\mathrm{P}_1}B = 20$}\\
\ref{Scheme3_30} \footnotesize {Scheme 3: $T_{\mathrm{P}_1}B = 40$}
}};

\end{tikzpicture}%

==> Figures_EPS/CE_PhaseII.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{every tick label/.append style={font=\footnotesize}}
\definecolor{ForestGreen}{RGB}{34,139,34}
\begin{tikzpicture}

\begin{axis}[%
width=0.95\textwidth,
height=0.45\textwidth,
at={(2,0.5)},
scale only axis,
xmin=16,
xmax=32,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize The number of pilots in Phase II ($T_{\mathrm{P}_2}$)},
ymode=log,
ymin=0.005,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize Normalized mean-square error},
yminorticks=true,
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids
]
\addplot [color=blue, line width=1.0pt, only marks, mark size=1.5pt, mark=*, mark options={solid, fill=blue, draw=blue}, forget plot]
  table[row sep=crcr]{%
8	0.0126584983703508\\
9	0.0123181574420604\\
10	0.0120442138793873\\
11	0.0119219492939443\\
12	0.0117978477733317\\
13	0.0114741297350817\\
14	0.0115957872457875\\
15	0.0115893915512486\\
16	0.0112662859339249\\
17	0.0110330800056879\\
18	0.0104916617939654\\
19	0.00992305467141384\\
20	0.00948036904296142\\
21	0.00915106599716136\\
22	0.00879224385982825\\
23	0.00849176368892956\\
24	0.00825497252006405\\
25	0.00793335375029911\\
26	0.00771127715033204\\
27	0.00747529066032171\\
28	0.00722070255103912\\
29	0.00700896876499528\\
30	0.00681769687910352\\
31	0.00661867932204116\\
32	0.00643495446094051\\
};\label{UE1_Num_Pro}
\addplot [color=blue, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
8	0.0128226454567009\\
9	0.0124652719062927\\
10	0.0123365574689706\\
11	0.012092764826973\\
12	0.0120123664665884\\
13	0.0117564744791109\\
14	0.0116466414715632\\
15	0.0115034012045304\\
16	0.0115424555873966\\
17	0.0109817764451667\\
18	0.0104770679456292\\
19	0.0100200148001973\\
20	0.00960390672320244\\
21	0.00922326456293437\\
22	0.00887356692588887\\
23	0.00855104702839695\\
24	0.00825253951607933\\
25	0.0079753634201541\\
26	0.00771723163830949\\
27	0.00747618015022373\\
28	0.00725051209954317\\
29	0.00703875320389314\\
30	0.00683961588839746\\
31	0.00665197020309993\\
32	0.0064748200641449\\
};\label{UE1_Ana_Pro}
\addplot [color=ForestGreen, line width=1.0pt, only marks, mark size=1.5pt, mark=*, mark options={solid, fill=ForestGreen, draw=ForestGreen}, forget plot]
  table[row sep=crcr]{%
8	0.0196971122150879\\
9	0.0197998954376477\\
10	0.0206055533113366\\
11	0.020203483449178\\
12	0.020211886932541\\
13	0.0183512891151071\\
14	0.0170092098139574\\
15	0.0148146211779162\\
16	0.0134302967757638\\
17	0.0127511019924304\\
18	0.0122668800325666\\
19	0.0116094379080843\\
20	0.0111429235284845\\
21	0.0108146940707323\\
22	0.0104313319156415\\
23	0.0100081150164386\\
24	0.00956996844471149\\
25	0.00939773526365877\\
26	0.00901688633345191\\
27	0.00877848169673597\\
28	0.00850018393784072\\
29	0.00819351255468818\\
30	0.00809343250271714\\
31	0.00762452830204365\\
32	0.00760726955999752\\
};\label{UE2_Num_Pro}
\addplot [color=ForestGreen, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
8	0.0188362661968962\\
9	0.0189746976852608\\
10	0.0199546704226755\\
11	0.0193388150382067\\
12	0.0194005991379007\\
13	0.0174500145654965\\
14	0.0161570802609436\\
15	0.0139678688243313\\
16	0.0124231315800523\\
17	0.0118165852080046\\
18	0.011272890078428\\
19	0.0107824045551923\\
20	0.0103373870055088\\
21	0.0099315478414631\\
22	0.00955972277003063\\
23	0.00921763062079256\\
24	0.00890169125104799\\
25	0.00860888681861461\\
26	0.00833665482259364\\
27	0.00808280472888157\\
28	0.00784545232170867\\
29	0.00762296752950741\\
30	0.00741393260088574\\
31	0.00721710830830861\\
32	0.00703140643454487\\
};\label{UE2_Ana_Pro}
\addplot [color=blue, line width=1.0pt, only marks, mark size=1.5pt, mark=*, mark options={solid, fill=blue, draw=blue}, forget plot]
  table[row sep=crcr]{%
8	0.279858798988092\\
9	0.273240239659704\\
10	0.257956011222487\\
11	0.252794442427138\\
12	0.253273715551003\\
13	0.256431103873641\\
14	0.26001682687839\\
15	0.264117240576723\\
16	0.277098212431205\\
17	0.263403703339592\\
18	0.252141510904642\\
19	0.245438298163394\\
20	0.235660407317838\\
21	0.222102435698058\\
22	0.213000279415628\\
23	0.207931638856313\\
24	0.198513260831645\\
25	0.19505014205597\\
26	0.188086611733665\\
27	0.181433663876585\\
28	0.174875993932523\\
29	0.172226022465661\\
30	0.167640360733263\\
31	0.160344505868167\\
32	0.157557873041669\\
};\label{UE1_Num_Pri}
\addplot [color=blue, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
8	0.269081784625898\\
9	0.258777669222429\\
10	0.251927120498677\\
11	0.248035847638399\\
12	0.246748986469669\\
13	0.24778677440716\\
14	0.25145834766454\\
15	0.257737371090619\\
16	0.267619386330284\\
17	0.255496980970869\\
18	0.244551606073482\\
19	0.23461261244838\\
20	0.225541559330758\\
21	0.21722485997774\\
22	0.209568369491966\\
23	0.202493339070616\\
24	0.195933348547042\\
25	0.189831950536262\\
26	0.184140839725784\\
27	0.178818414862058\\
28	0.17382863797004\\
29	0.169140121075987\\
30	0.164725388867821\\
31	0.160560278722306\\
32	0.156623448941212\\
};\label{UE1_Ana_Pri}
\addplot [color=ForestGreen, only marks, mark size=1.5pt, mark=*, mark options={solid, fill=ForestGreen, draw=ForestGreen}, forget plot]
  table[row sep=crcr]{%
8	0.0759870044454509\\
9	0.0758587753814575\\
10	0.0792995782316712\\
11	0.078631954653282\\
12	0.0774076633756972\\
13	0.0721679840495511\\
14	0.0665083300817716\\
15	0.0580977525826269\\
16	0.0536321428924009\\
17	0.0505030677708188\\
18	0.0486648292249604\\
19	0.04749884234209\\
20	0.0447617636732959\\
21	0.0441617649589728\\
22	0.0421651675388122\\
23	0.0415137039736642\\
24	0.0406757242138674\\
25	0.0385311840145513\\
26	0.0372887163338631\\
27	0.0374513158985309\\
28	0.0363284171511091\\
29	0.0352271020771069\\
30	0.034170569084539\\
31	0.033544641616396\\
32	0.0330288283660004\\
};\label{UE2_Num_Pri}
\addplot [color=ForestGreen, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
8	0.0855984442685094\\
9	0.0862884449728933\\
10	0.0902625691874269\\
11	0.0878892121931493\\
12	0.0881588624884551\\
13	0.0803208448366768\\
14	0.0749540932230648\\
15	0.0655422364299632\\
16	0.0585454092344764\\
17	0.0559638287258679\\
18	0.0536292734770248\\
19	0.0515062259597289\\
20	0.0495658237238025\\
21	0.0477843514165665\\
22	0.0461421277563113\\
23	0.0446226713902367\\
24	0.0432120670582342\\
25	0.0418984778646973\\
26	0.0406717656378675\\
27	0.0395231922887638\\
28	0.0384451825947568\\
29	0.03743113407599\\
30	0.0364752633441803\\
31	0.0355724809650665\\
32	0.0347182888081242\\
};\label{UE2_Ana_Pri}
\addplot [color=blue, line width=1.0pt, only marks, mark size=3pt, mark=+, mark options={solid, fill=blue, draw=blue}, forget plot]
  table[row sep=crcr]{%
8	0.0119631719503728\\
9	0.0115196629574925\\
10	0.0112738605256739\\
11	0.0112359597866944\\
12	0.0110330751407115\\
13	0.0109160722713047\\
14	0.0108832146181338\\
15	0.01099573880757\\
16	0.0109273460604425\\
17	0.0105767172623452\\
18	0.00996752865815106\\
19	0.00951220330924956\\
20	0.00905685825811242\\
21	0.00873353681524623\\
22	0.0083926397903074\\
23	0.00812420115337639\\
24	0.00789345254720283\\
25	0.00754484546129273\\
26	0.00733814590585926\\
27	0.00712301567315664\\
28	0.00689623167378549\\
29	0.00677907206521859\\
30	0.0065496487272678\\
31	0.00636677893015373\\
32	0.00619028355502416\\
};\label{UE1_Num_mis40}
\addplot [color=ForestGreen, line width=1.0pt, only marks, mark size=3pt, mark=+, mark options={solid, fill=ForestGreen, draw=ForestGreen}, forget plot]
  table[row sep=crcr]{%
8	0.0194223990943298\\
9	0.019258369016598\\
10	0.0204999695020757\\
11	0.0196531966472651\\
12	0.0197170829059668\\
13	0.0179920576699688\\
14	0.0165079799657827\\
15	0.0145661668252791\\
16	0.012972111161191\\
17	0.0122473654800311\\
18	0.0117812412912786\\
19	0.0113269836635173\\
20	0.0106394689711179\\
21	0.0103428609503804\\
22	0.00995217141670604\\
23	0.00964895899251178\\
24	0.00933194014634674\\
25	0.00888400762053414\\
26	0.00872629073496954\\
27	0.00841808120087441\\
28	0.00817320906831068\\
29	0.00792320973963359\\
30	0.0077302449313162\\
31	0.00753751067524736\\
32	0.00732976064451471\\
};\label{UE2_Num_mis40}
\end{axis}
\node (Box11) [draw=none,fill=white] at (5.9, 5.3) {\shortstack[l]{ 
\hspace{11.1cm} \\
\hspace{11.1cm} \\
\hspace{11.1cm} \\
\hspace{11.1cm} \\
\hspace{11.1cm} \\
\hspace{11.1cm} 
}};

\node (Box1) [draw=none,fill=none] at (1.72, 5.3) {\shortstack[l]{ 
\ref{UE1_Ana_Pri} \footnotesize {Analytical: UE1}\\
\ref{UE2_Ana_Pri} \footnotesize {Analytical: UE2}
}};

\node (Box1) [draw=none,fill=none] at (5.12, 5.3) {\shortstack[l]{ \ref{UE1_Num_Pri} \footnotesize {Numerical: UE1} \\
\ref{UE2_Num_Pri} \footnotesize {Numerical: UE2}
}};

\node (Box1) [draw=none,fill=none] at (9.32, 5.3) {\shortstack[l]{ \ref{UE1_Num_mis40} \footnotesize {Numerical: mismatched $\kappa$, UE1} \\
\ref{UE2_Num_mis40} \footnotesize {Numerical: mismatched $\kappa$, UE2}
}};

\draw [black] (2, 1.5) ellipse [x radius=0.16, y radius=0.5];
\draw[-{Stealth}, color=black] (2.95, 1.7) -- (2.15,1.7);
\node (lab1) at (3.9, 1.7) {\footnotesize With Phase I};

\draw [black] (0.9, 3.7) ellipse [x radius=0.16, y radius=1.2];
\draw[-{Stealth}, color=black] (1.9, 3.7) -- (1.1,3.7);
\node (lab1) at (3.0, 3.7) {\footnotesize Without Phase I};
\end{tikzpicture}%

==> Figures_EPS/RISLoc.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor2}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor3}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor4}{rgb}{0.63500,0.07800,0.18400}%
%
\pgfplotsset{every tick label/.append style={font=\footnotesize}}

\begin{tikzpicture}

\begin{axis}[%
width=0.95\textwidth,
height=0.45\textwidth,
at={(2,0.5)},
scale only axis,
xmin=7,
xmax=22,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Transmission Power (dBm)},
ymode=log,
ymin=0.001,
ymax=10,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize RMSE (m)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	0.0492999067020729\\
5	0.0407339227336556\\
7	0.0342438355934864\\
9	0.0294212294787311\\
11	0.0259207435052718\\
13	0.0234446900031895\\
15	0.0217377702487971\\
17	0.0205880896850028\\
19	0.0198284211087611\\
21	0.0193337503772278\\
22	0.0191567691035665\\
};\label{PEB_Kappa5T40UE1}
\addplot [color=blue, only marks, mark = o, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	1.58355307529454\\
5	0.0399761780197812\\
7	0.0333433472765372\\
9	0.0285195818532644\\
11	0.0250622954479903\\
13	0.0226317129992102\\
15	0.0209599209746118\\
17	0.0198434050809991\\
19	0.0191017757966622\\
21	0.0186197583212193\\
22	0.018445989447321\\
};\label{RMSE_Kappa5T40UE1}
\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	0.140033432872213\\
5	0.114147862713133\\
7	0.0942245727125272\\
9	0.0791130400884035\\
11	0.0678685887768154\\
13	0.0596937569430941\\
15	0.0539015940578863\\
17	0.0499022584265417\\
19	0.0472048270517588\\
21	0.0454205121067472\\
22	0.0447761814192436\\
};\label{PEB_Kappa5T40UE2}
\addplot [color=blue, only marks, mark = o, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	16.1666589628815\\
5	17.2469645640947\\
7	6.69135528517555\\
9	3.37529951818009\\
11	2.17253319708339\\
13	0.0644909751744742\\
15	0.0581479496576689\\
17	0.0537939636447807\\
19	0.0508471929931626\\
21	0.0489160554347135\\
22	0.0482069631438435\\
};\label{RMSE_Kappa5T40UE2}
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	0.0425488445552815\\
5	0.0339832324001424\\
7	0.027225718117472\\
9	0.0219149018869698\\
11	0.0177650695064094\\
13	0.0145499470179511\\
15	0.0120891087083558\\
17	0.0102364307074018\\
19	0.0088705599258325\\
21	0.00788798519160567\\
22	0.00751199203910897\\
};\label{PEB_Kappa50T40UE1}
\addplot [color=red, only marks, mark = o, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	0.0418687730011746\\
5	0.0330823421184159\\
7	0.02634665097217\\
9	0.0211309694856031\\
11	0.0170931284909413\\
13	0.0139831453049001\\
15	0.0116129199204914\\
17	0.00982750804235339\\
19	0.00851398342891327\\
21	0.00756988070044341\\
22	0.00720577535121826\\
};\label{RMSE_Kappa50T40UE1}
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	0.123824947616358\\
5	0.0986911042404208\\
7	0.0788110986215984\\
9	0.0631244946414517\\
11	0.0507925508287064\\
13	0.0411521883233169\\
15	0.0336783943233301\\
17	0.0279528131888846\\
19	0.0236370687893448\\
21	0.020450651836727\\
22	0.0192049508624571\\
};\label{PEB_Kappa50T40UE2}
\addplot [color=red, only marks, mark = o, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
3	17.8669641405913\\
5	7.55423997324125\\
7	5.76886355050308\\
9	2.67659739065052\\
11	0.0547570670615259\\
13	0.0442906362717921\\
15	0.0361984486718277\\
17	0.0300385620020511\\
19	0.0253995111025362\\
21	0.0219784768912881\\
22	0.0206377949024042\\
};\label{RMSE_Kappa50T40UE2}

\end{axis}

\node (Box1) [draw=none,fill=white] at (10, 4.8) {\shortstack[l]{ 
\ref{PEB_Kappa5T40UE1} \footnotesize PEB, \textit{$\kappa = 5$} \\
\ref{RMSE_Kappa5T40UE1} \footnotesize \hspace{5.1mm} RMSE, \textit{$\kappa = 5$} \\
\ref{PEB_Kappa50T40UE1} \footnotesize PEB, \textit{$\kappa = 50$} \\
\ref{RMSE_Kappa50T40UE1} \footnotesize \hspace{4.3mm} RMSE, \textit{$\kappa = 50$}
}};
\draw [black] (2.3, 2.1) ellipse [x radius=0.1, y radius=0.4];
\draw[-{Stealth}, color=black] (1.61, 1.9) -- (2.21,1.9);
\node (lab1) at (1.3, 1.9) {\footnotesize UE1};
\draw [black] (1.3, 3.0) ellipse [x radius=0.1, y radius=0.4];
\draw[-{Stealth}, color=black] (2, 3.2) -- (1.39, 3.2);
\node (lab2) at (2.3, 3.2) {\footnotesize UE2};
\end{tikzpicture}%

==> Figures_EPS/Rate_CE.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\pgfplotsset{every tick label/.append style={font=\footnotesize}}

\begin{tikzpicture}

\begin{axis}[%
width=0.95\textwidth,
height=0.45\textwidth,
at={(2,1)},
scale only axis,
xmin=9,
xmax=96,
xlabel style={font=\color{white!15!black}},
xlabel={\footnotesize Number of pilots in Phase II},
ymin=0,
ymax=5,
ylabel style={font=\color{white!15!black}},
ylabel={\footnotesize Effective achievable rate (bits/s/Hz)},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=black, dotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	2.29739899285233\\
13	2.74261332100361\\
14	2.91827308493004\\
15	3.04158532225264\\
16	3.11435581076696\\
17	3.11616251839356\\
18	3.10848586089295\\
19	3.10061051446086\\
20	3.08195457149784\\
24	3.03774906149494\\
32	2.85893862344843\\
40	2.66079362768031\\
48	2.43438149838136\\
56	2.18902529173401\\
64	1.93583487303659\\
72	1.67469627109929\\
80	1.40554667580863\\
88	1.13080120598923\\
96	0.85201822487754\\
};\label{Rate_Pri}
\addplot [color=black, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	3.84730456964682\\
13	3.9351336158378\\
14	4.00556495872528\\
15	4.07464050097448\\
16	4.10646314360733\\
17	4.09078077606483\\
18	4.06364340796484\\
19	4.02580367200851\\
20	3.99459957066797\\
24	3.88430624753224\\
32	3.59747437201779\\
40	3.29727758697569\\
48	2.99416855218823\\
56	2.68031971810579\\
64	2.34749388445851\\
72	2.01960569411296\\
80	1.68836320809273\\
88	1.35060092780324\\
96	1.01941433405454\\
};\label{Rate_CHest}
\addplot [color=black, dashdotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	4.82346974742195\\
13	4.69192057249227\\
14	4.64807084751572\\
15	4.60422112253913\\
16	4.56037139756262\\
17	4.51652167258604\\
18	4.4726719476095\\
19	4.42882222263288\\
20	4.38497249765629\\
24	4.20957359775009\\
32	3.85877579793758\\
40	3.50797799812507\\
48	3.15718019831255\\
56	2.80638239850009\\
64	2.45558459868755\\
72	2.10478679887503\\
80	1.75398899906253\\
88	1.40319119925005\\
96	1.05239339943751\\
};\label{Rate_Perf}
\addplot [color=black, dotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	1.59449414290457\\
13	1.98151334349348\\
14	2.14136034757978\\
15	2.26319414583589\\
16	2.37330740175776\\
19	2.37771133039635\\
20	2.36212717133426\\
24	2.32136951064815\\
32	2.23538917485567\\
40	2.09564890966848\\
48	1.92575366652376\\
56	1.73702202272042\\
64	1.54006412450688\\
72	1.33701368980167\\
80	1.12436810635034\\
88	0.903827695241538\\
96	0.685210805653173\\
};\label{Rate_PriKappa5}
\addplot [color=black, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	2.87555207486242\\
13	3.14332157339995\\
14	3.25915926667747\\
15	3.36945872683891\\
16	3.45014796379594\\
17	3.44128582157648\\
18	3.43524859945848\\
19	3.42683639972834\\
20	3.40865708884132\\
24	3.33845381668774\\
32	3.13179598207287\\
40	2.90590199284454\\
48	2.65105187876965\\
56	2.38732257395965\\
64	2.10526798788649\\
72	1.81935437457936\\
80	1.52561557266191\\
88	1.229102937472\\
96	0.926999625967145\\
};\label{Rate_CHestKappa5}
\addplot [color=black, dashdotted, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
10	4.53093781493692\\
13	4.40736678362044\\
14	4.36617643984831\\
15	4.32498609607613\\
16	4.28379575230404\\
17	4.24260540853185\\
18	4.20141506475962\\
19	4.16022472098745\\
20	4.1190343772153\\
24	3.95427300212676\\
32	3.62475025194955\\
40	3.29522750177227\\
48	2.96570475159509\\
56	2.6361820014178\\
64	2.3066592512406\\
72	1.97713650106335\\
80	1.64761375088615\\
88	1.31809100070892\\
96	0.988568250531671\\
};\label{Rate_Perfkappa5}
\end{axis}

\node (Box1) [draw=none,fill=white] at (8, 4.7) {\shortstack[l]{ 
\ref{Rate_Pri} \footnotesize {Without Phase I, estimated channel}\\
\ref{Rate_CHest} \footnotesize {With Phase I, estimated channel}\\
\ref{Rate_Perf} \footnotesize {With Phase I, perfect channel}
}};

\draw[-{Stealth}, color=blue] (3.5, 0.95) -- (2.3,4.15);
\draw[-{Stealth}, color=blue] (3.5, 0.95) -- (4,3.91);
\draw[-{Stealth}, color=blue] (3.5, 0.95) -- (5,2.68);
\node (lab1) at (3.5, 0.75) {\footnotesize \textcolor{blue}{$\kappa = 50$}};

\draw[-{Stealth}, color=red] (2, 0.95) -- (0.6,4.8);
\draw[-{Stealth}, color=red] (2, 0.95) -- (2.2,3.6);
\draw[-{Stealth}, color=red] (2, 0.95) -- (0.63,2.2);
\node (lab1) at (2, 0.75) {\footnotesize \textcolor{red}{$\kappa = 5$}};
\end{tikzpicture}%

==> Figures_EPS/packages.tex <==
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts,steinmetz}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{tikz}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
    
    
%packages
\usepackage{pgfplots}
\usepackage[font=footnotesize]{caption}
\usepackage{subcaption}
\usepackage{bbm}
%\usepackage{bm}

\usetikzlibrary{calc}
\makeatletter
\newcommand{\gettikzxy}[3]{%
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
  \edef#2{\the\pgf@x}%
  \edef#3{\the\pgf@y}%
}
\makeatother
% \usepackage[disable]{todonotes} % notes not showed
\usepackage[draft]{todonotes}   % notes showed
\usepackage{upgreek} %use for mathbf symbols like \bm{theta} = \mathbf{\uptheta}
\usepackage{seqsplit}

\usetikzlibrary{arrows.meta,arrows}
\usepackage[]{algorithm}
\usepackage[noend]{algpseudocode}

